Hybrid Reinforcement Learning and Model Predictive Control for Adaptive Control of Hydrogen-Diesel Dual-Fuel Combustion

Reinforcement Learning (RL) and Machine Learning Integrated Model Predictive Control (ML-MPC) are promising approaches for optimizing hydrogen-diesel dual-fuel engine control, as they can effectively control multiple-input multiple-output systems and nonlinear processes. ML-MPC is advantageous for providing safe and optimal controls, ensuring the engine operates within predefined safety limits. In contrast, RL is distinguished by its adaptability to changing conditions through its learning-based approach. However, the practical implementation of either method alone poses challenges. RL requires high variance in control inputs during early learning phases, which can pose risks to the system by potentially executing unsafe actions, leading to mechanical damage. Conversely, ML-MPC relies on an accurate system model to generate optimal control inputs and has limited adaptability to system drifts, such as injector aging, which naturally occur in engine applications. To address these limitations, this study proposes a hybrid RL and ML-MPC approach that uses an ML-MPC framework while incorporating an RL agent to dynamically adjust the ML-MPC load tracking reference in response to changes in the environment. At the same time, the ML-MPC ensures that actions stay safe throughout the RL agent's exploration. To evaluate the effectiveness of this approach, fuel pressure is deliberately varied to introduce a model-plant mismatch between the ML-MPC and the engine test bench. The result of this mismatch is a root mean square error (RMSE) in indicated mean effective pressure of 0.57 bar when running the ML-MPC. The experimental results demonstrate that RL successfully adapts to changing boundary conditions by altering the tracking reference while ML-MPC ensures safe control inputs. The quantitative improvement in load tracking by implementing RL is an RSME of 0.44 bar.

==> Figures/PlotEpisodeValidation.tex <==
\begin{tikzpicture}
\setlength{\PlotWidth}{6.7cm} 
\setlength{\PlotHeight}{1.7cm} 
\setlength{\DeltaHeight}{0.4cm}
\setlength{\DeltaHeightDashed}{0.2cm}
\setlength{\DeltaWidth}{0.9cm}

\newcommand{\NumPlotY}{1}
\newcommand{\NumPlotX}{1}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\pgfmathsetlength{\Xpos}{(\NumPlotX-1)*\PlotWidth +(\NumPlotX-1)*\NumPlotX*\DeltaWidth}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ymin=3.5,
	ymax=10,
	ylabel style={at={(-0.1,0.5)}},
    ylabel={\shortstack {IMEP / \\ \si{\bar}}},
    axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0,1.2)},legend columns=5, legend cell align=left, align=left, anchor=south west,  draw=none,fill=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	legend style={font=\scriptsize}
	]
	%Dummies for legend
	\addplot[ color=mmpDarkBlue,line width=1pt] table {
		x y 
		0 1
		1 1
	};
    %\addplot[ color=mmpBlack,line width=1pt] table {
	%	x y 
	%	0 1
	%	1 1
	%};
	\addplot[ color=mmpLightBlue,line width=1pt] table {
		x y 
		0 1
		1 1
	};
	\addplot[ color=mmpRed,line width=1pt] table {
		x y 
		0 1
		1 1
	};
    \addplot[ color=mmpOrange,line width=1pt] table {
		x y 
		0 1
		1 1
	};
	
	\addplot[ color=mmpRed,line width=0.5pt,forget plot] table [x index=0, y index=1, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};

   \addplot[ color=mmpOrange,line width=0.5pt,forget plot] table [x index=0, y index=12, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};
   
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=2, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};

    %\addplot[ color=mmpBlack,line width=0.5pt, forget plot] table [x index=0, y index=2, col sep=comma] {Figures/Data/DataRLVSR4_episode1.csv};

	\addplot[ color=mmpLightBlue,line width=0.5pt,forget plot] table [x index=0, y index=8, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};


    
	\addlegendentry{Measured RL converged}
    %\addlegendentry{Measured RL Episode 1}
	\addlegendentry{MPC Prediction}
	\addlegendentry{Reference}
    \addlegendentry{RL2MPC Reference}
	
\end{axis}

\renewcommand{\NumPlotY}{2}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack {MPRR / \\$\frac{\si{\bar}}{\si{\degreeKW}}$}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.02,2.6)},legend columns=3, legend cell align=left, align=left, anchor=north west, draw=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	
    \addplot[ color=mmpDarkBlue,line width=0.5pt, forget plot] table [x index=0, y index=3, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};

    \addplot[ color=mmpDarkBlue,line width=0.5pt, forget plot] table [x index=0, y index=3, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};

    %\addplot[ color=mmpBlack,line width=0.5pt, forget plot] table [x index=0, y index=3, col sep=comma] {Figures/Data/DataRLVSR4_episode1.csv};

    
    \addplot[ color=mmpLightBlue,line width=0.5pt, forget plot] table [x index=0, y index=9, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};


    
    
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
\end{axis}

\renewcommand{\NumPlotY}{3}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	ymin=0,
	ymax=1500,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack { NOx /  \\ ppm}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.02,2.6)},legend columns=2, legend cell align=left, align=left, anchor=north west, draw=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	 	
    \addplot[ color=mmpDarkBlue,line width=0.5pt, forget plot] table [x index=0, y index=14, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};
    %\addplot[ color=mmpBlack,line width=0.5pt, forget plot] table [x index=0, y index=14, col sep=comma] {Figures/Data/DataRLVSR4_episode1.csv};
    \addplot[ color=mmpLightBlue,line width=0.5pt, forget plot] table [x index=0, y index=10, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};
	
\end{axis}

\renewcommand{\NumPlotY}{4}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xlabel style={font=\color{white!15!black}},
	xlabel={Cycle / -},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack {Soot / \\ $\frac{\si{\milli\gram}}{\si{\cubic\meter}}$}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.02,0.05)},legend columns=2, legend cell align=left, align=left, anchor=south west, draw=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
    
    \addplot[ color=mmpDarkBlue,line width=0.5pt, forget plot] table [x index=0, y index=15, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};
    %\addplot[ color=mmpBlack,line width=0.5pt, forget plot] table [x index=0, y index=15, col sep=comma] {Figures/Data/DataRLVSR4_episode1.csv};
    \addplot[ color=mmpLightBlue,line width=0.5pt, forget plot] table [x index=0, y index=11, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};

\end{axis}

%\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*(\NumPlotY)*\DeltaHeight-\DeltaHeightDashed/2-\DeltaHeight/2}
%\pgfmathsetlength{\XEndPos}{\PlotWidth+0.5cm}


%node position
%\pgfmathsetlength{\Ypos}{-1*\NumPlotY/2*\PlotHeight - 1*\NumPlotY/2*\DeltaHeight-\DeltaHeightDashed/4-\DeltaHeight/4}
%\node[rotate=270] at (\XEndPos-0.05cm,\Ypos) {\scriptsize States/Objectives};

%node position
%\pgfmathsetlength{\Ypos}{-1*6*\PlotHeight - 1*6*\DeltaHeight-\DeltaHeightDashed+\PlotHeight/2}
%\node[rotate=270] at (\XEndPos-0.05cm,\Ypos) {\scriptsize Actions};

%curly bracket
%\pgfmathsetlength{\YposTop}{-\DeltaHeight}
%\pgfmathsetlength{\YposButtom}{-1*4*\PlotHeight - 1*4*\DeltaHeight}
%\draw[thick,black,decorate,decoration={brace,amplitude=6pt}]  (\XEndPos-0.45cm,\YposTop)-- (\XEndPos-0.45cm,\YposButtom);

%curly bracket
%\pgfmathsetlength{\YposTop}{{-1*4*\PlotHeight - 1*5*\DeltaHeight}
%\pgfmathsetlength{\YposButtom}{-1*7*\PlotHeight - 1*7*\DeltaHeight
%\draw[thick,black,decorate,decoration={brace,amplitude=6pt}]  (\XEndPos-0.45cm,\YposTop)-- (\XEndPos-0.45cm,\YposButtom);

%\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*(\NumPlotY)*\DeltaHeight-\DeltaHeightDashed/2-\DeltaHeight/2}
%\pgfmathsetlength{\XEndPos}{\PlotWidth+0.35cm}
%\draw[dashed,thick] (-0.75cm,\Ypos) -- (\XEndPos,\Ypos);

\renewcommand{\NumPlotY}{1}
\renewcommand{\NumPlotX}{2}
\pgfmathsetlength{\Xpos}{(\NumPlotX-1)*\PlotWidth +(\NumPlotX-1)*\NumPlotX*\DeltaWidth}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack  {DOI Main / \\ \si{\second}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=4, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};
	
\end{axis}

\renewcommand{\NumPlotY}{2}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack { P2M / \\ \si{\micro\second}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=6, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};
\end{axis}

\renewcommand{\NumPlotY}{3}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={ \shortstack  { SOI Main / \\ \si{\degreeKWbZOT}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=7, col sep=comma] {Figures/Data/DataRLVSR10_episode21.csv};
\end{axis}



\renewcommand{\NumPlotY}{4}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xlabel style={font=\color{white!15!black}},
	xlabel={Cycle / -},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack  {DOI H2 / \\ \si{\second}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	%\addplot[ area legend, draw=black, fill=blue, opacity=0.5]
	%	table[x index=0, y index=1, col sep=comma]{Figures/Data/PlotEpisode/LimitsRLVSR30089_episode114.csv};
	
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=5, col sep=comma]		 {Figures/Data/DataRLVSR10_episode21.csv};
\end{axis}




\end{tikzpicture}


==> Figures/PlotMPCAfterMismatch.tex <==
\begin{tikzpicture}
\setlength{\PlotWidth}{6.7cm} 
\setlength{\PlotHeight}{1.7cm} 
\setlength{\DeltaHeight}{0.4cm}
\setlength{\DeltaHeightDashed}{0.2cm}
\setlength{\DeltaWidth}{0.9cm}

\newcommand{\NumPlotY}{1}
\newcommand{\NumPlotX}{1}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\pgfmathsetlength{\Xpos}{(\NumPlotX-1)*\PlotWidth +(\NumPlotX-1)*\NumPlotX*\DeltaWidth}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ymin=3.5,
	ymax=9.5,
	ylabel style={at={(-0.1,0.5)}},
    ylabel={\shortstack {IMEP / \\ \si{\bar}}},
    axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.5,1.25)},legend columns=3, legend cell align=left, align=left, anchor=center,  draw=none,fill=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	legend style={font=\scriptsize}
	]
	%Dummies for legend
	\addplot[ color=mmpDarkBlue,line width=1pt] table {
		x y 
		0 1
		1 1
	};
	\addplot[ color=mmpLightBlue,line width=1pt] table {
		x y 
		0 1
		1 1
	};
	\addplot[ color=mmpRed,line width=1pt] table {
		x y 
		0 1
		1 1
	};
	
	\addplot[ color=mmpRed,line width=0.5pt,forget plot] table [x index=0, y index=1, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};

   
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=2, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};

	\addplot[ color=mmpLightBlue,line width=0.5pt,forget plot] table [x index=0, y index=8, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};


    
	\addlegendentry{Measured}
	\addlegendentry{MPC Prediction}
	\addlegendentry{Reference}
    \addlegendentry{RL2MPC Reference}
	
\end{axis}

\renewcommand{\NumPlotY}{2}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack {MPRR / \\$\frac{\si{\bar}}{\si{\degreeKW}}$}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.02,2.6)},legend columns=3, legend cell align=left, align=left, anchor=north west, draw=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	
    \addplot[ color=mmpDarkBlue,line width=0.5pt, forget plot] table [x index=0, y index=3, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};
    \addplot[ color=mmpLightBlue,line width=0.5pt, forget plot] table [x index=0, y index=9, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};
    
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
\end{axis}

\renewcommand{\NumPlotY}{3}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	ymin=0,
	ymax=1500,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack { NOx /  \\ ppm}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.02,2.6)},legend columns=2, legend cell align=left, align=left, anchor=north west, draw=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	 	
    \addplot[ color=mmpDarkBlue,line width=0.5pt, forget plot] table [x index=0, y index=13, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};
    \addplot[ color=mmpLightBlue,line width=0.5pt, forget plot] table [x index=0, y index=10, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};
	
\end{axis}

\renewcommand{\NumPlotY}{4}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xlabel style={font=\color{white!15!black}},
	xlabel={Cycle / -},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack {Soot / \\ $\frac{\si{\milli\gram}}{\si{\cubic\meter}}$}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.02,0.05)},legend columns=2, legend cell align=left, align=left, anchor=south west, draw=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
    
    \addplot[ color=mmpDarkBlue,line width=0.5pt, forget plot] table [x index=0, y index=14, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};
    \addplot[ color=mmpLightBlue,line width=0.5pt, forget plot] table [x index=0, y index=11, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};

\end{axis}

%\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*(\NumPlotY)*\DeltaHeight-\DeltaHeightDashed/2-\DeltaHeight/2}
%\pgfmathsetlength{\XEndPos}{\PlotWidth+0.5cm}


%node position
%\pgfmathsetlength{\Ypos}{-1*\NumPlotY/2*\PlotHeight - 1*\NumPlotY/2*\DeltaHeight-\DeltaHeightDashed/4-\DeltaHeight/4}
%\node[rotate=270] at (\XEndPos-0.05cm,\Ypos) {\scriptsize States/Objectives};

%node position
%\pgfmathsetlength{\Ypos}{-1*6*\PlotHeight - 1*6*\DeltaHeight-\DeltaHeightDashed+\PlotHeight/2}
%\node[rotate=270] at (\XEndPos-0.05cm,\Ypos) {\scriptsize Actions};

%curly bracket
%\pgfmathsetlength{\YposTop}{-\DeltaHeight}
%\pgfmathsetlength{\YposButtom}{-1*4*\PlotHeight - 1*4*\DeltaHeight}
%\draw[thick,black,decorate,decoration={brace,amplitude=6pt}]  (\XEndPos-0.45cm,\YposTop)-- (\XEndPos-0.45cm,\YposButtom);

%curly bracket
%\pgfmathsetlength{\YposTop}{{-1*4*\PlotHeight - 1*5*\DeltaHeight}
%\pgfmathsetlength{\YposButtom}{-1*7*\PlotHeight - 1*7*\DeltaHeight
%\draw[thick,black,decorate,decoration={brace,amplitude=6pt}]  (\XEndPos-0.45cm,\YposTop)-- (\XEndPos-0.45cm,\YposButtom);

%\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*(\NumPlotY)*\DeltaHeight-\DeltaHeightDashed/2-\DeltaHeight/2}
%\pgfmathsetlength{\XEndPos}{\PlotWidth+0.35cm}
%\draw[dashed,thick] (-0.75cm,\Ypos) -- (\XEndPos,\Ypos);

\renewcommand{\NumPlotY}{1}
\renewcommand{\NumPlotX}{2}
\pgfmathsetlength{\Xpos}{(\NumPlotX-1)*\PlotWidth +(\NumPlotX-1)*\NumPlotX*\DeltaWidth}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack  {DOI Main / \\ \si{\second}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=4, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};
	
\end{axis}

\renewcommand{\NumPlotY}{2}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack { P2M / \\ \si{\micro\second}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=6, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};
\end{axis}

\renewcommand{\NumPlotY}{3}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={ \shortstack  { SOI Main / \\ \si{\degreeKWbZOT}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=7, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0006.csv};
\end{axis}



\renewcommand{\NumPlotY}{4}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xlabel style={font=\color{white!15!black}},
	xlabel={Cycle / -},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack  {DOI H2 / \\ \si{\second}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	%\addplot[ area legend, draw=black, fill=blue, opacity=0.5]
	%	table[x index=0, y index=1, col sep=comma]{Figures/Data/PlotEpisode/LimitsRLVSR30089_episode114.csv};
	
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=5, col sep=comma]		 {Figures/Data/MPCData_MCRL_0010MP0006.csv};
\end{axis}




\end{tikzpicture}


==> Figures/PlotMPCBeforeMismatch.tex <==
\begin{tikzpicture}
\setlength{\PlotWidth}{6.7cm} 
\setlength{\PlotHeight}{1.7cm} 
\setlength{\DeltaHeight}{0.4cm}
\setlength{\DeltaHeightDashed}{0.2cm}
\setlength{\DeltaWidth}{0.9cm}

\newcommand{\NumPlotY}{1}
\newcommand{\NumPlotX}{1}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\pgfmathsetlength{\Xpos}{(\NumPlotX-1)*\PlotWidth +(\NumPlotX-1)*\NumPlotX*\DeltaWidth}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ymin=3.5,
	ymax=9.5,
	ylabel style={at={(-0.1,0.5)}},
    ylabel={\shortstack {IMEP / \\ \si{\bar}}},
    axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.5,1.25)},legend columns=3, legend cell align=left, align=left, anchor=center,  draw=none,fill=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	legend style={font=\scriptsize}
	]
	%Dummies for legend
	\addplot[ color=mmpDarkBlue,line width=1pt] table {
		x y 
		0 1
		1 1
	};
	\addplot[ color=mmpLightBlue,line width=1pt] table {
		x y 
		0 1
		1 1
	};
	\addplot[ color=mmpRed,line width=1pt] table {
		x y 
		0 1
		1 1
	};
	
	\addplot[ color=mmpRed,line width=0.5pt,forget plot] table [x index=0, y index=1, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};

   
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=2, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};

	\addplot[ color=mmpLightBlue,line width=0.5pt,forget plot] table [x index=0, y index=8, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};


    
	\addlegendentry{Measured}
	\addlegendentry{MPC Prediction}
	\addlegendentry{Reference}
    \addlegendentry{RL2MPC Reference}
	
\end{axis}

\renewcommand{\NumPlotY}{2}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack {MPRR / \\$\frac{\si{\bar}}{\si{\degreeKW}}$}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.02,2.6)},legend columns=3, legend cell align=left, align=left, anchor=north west, draw=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	
    \addplot[ color=mmpDarkBlue,line width=0.5pt, forget plot] table [x index=0, y index=3, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};
    \addplot[ color=mmpLightBlue,line width=0.5pt, forget plot] table [x index=0, y index=9, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};
    
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
\end{axis}

\renewcommand{\NumPlotY}{3}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	ymin=0,
	ymax=1500,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack { NOx /  \\ ppm}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.02,2.6)},legend columns=2, legend cell align=left, align=left, anchor=north west, draw=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	 	
    \addplot[ color=mmpDarkBlue,line width=0.5pt, forget plot] table [x index=0, y index=13, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};
    \addplot[ color=mmpLightBlue,line width=0.5pt, forget plot] table [x index=0, y index=10, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};
	
\end{axis}

\renewcommand{\NumPlotY}{4}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xlabel style={font=\color{white!15!black}},
	xlabel={Cycle / -},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack {Soot / \\ $\frac{\si{\milli\gram}}{\si{\cubic\meter}}$}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.02,0.05)},legend columns=2, legend cell align=left, align=left, anchor=south west, draw=none},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
    
    \addplot[ color=mmpDarkBlue,line width=0.5pt, forget plot] table [x index=0, y index=14, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};
    \addplot[ color=mmpLightBlue,line width=0.5pt, forget plot] table [x index=0, y index=11, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};

\end{axis}

%\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*(\NumPlotY)*\DeltaHeight-\DeltaHeightDashed/2-\DeltaHeight/2}
%\pgfmathsetlength{\XEndPos}{\PlotWidth+0.5cm}


%node position
%\pgfmathsetlength{\Ypos}{-1*\NumPlotY/2*\PlotHeight - 1*\NumPlotY/2*\DeltaHeight-\DeltaHeightDashed/4-\DeltaHeight/4}
%\node[rotate=270] at (\XEndPos-0.05cm,\Ypos) {\scriptsize States/Objectives};

%node position
%\pgfmathsetlength{\Ypos}{-1*6*\PlotHeight - 1*6*\DeltaHeight-\DeltaHeightDashed+\PlotHeight/2}
%\node[rotate=270] at (\XEndPos-0.05cm,\Ypos) {\scriptsize Actions};

%curly bracket
%\pgfmathsetlength{\YposTop}{-\DeltaHeight}
%\pgfmathsetlength{\YposButtom}{-1*4*\PlotHeight - 1*4*\DeltaHeight}
%\draw[thick,black,decorate,decoration={brace,amplitude=6pt}]  (\XEndPos-0.45cm,\YposTop)-- (\XEndPos-0.45cm,\YposButtom);

%curly bracket
%\pgfmathsetlength{\YposTop}{{-1*4*\PlotHeight - 1*5*\DeltaHeight}
%\pgfmathsetlength{\YposButtom}{-1*7*\PlotHeight - 1*7*\DeltaHeight
%\draw[thick,black,decorate,decoration={brace,amplitude=6pt}]  (\XEndPos-0.45cm,\YposTop)-- (\XEndPos-0.45cm,\YposButtom);

%\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*(\NumPlotY)*\DeltaHeight-\DeltaHeightDashed/2-\DeltaHeight/2}
%\pgfmathsetlength{\XEndPos}{\PlotWidth+0.35cm}
%\draw[dashed,thick] (-0.75cm,\Ypos) -- (\XEndPos,\Ypos);

\renewcommand{\NumPlotY}{1}
\renewcommand{\NumPlotX}{2}
\pgfmathsetlength{\Xpos}{(\NumPlotX-1)*\PlotWidth +(\NumPlotX-1)*\NumPlotX*\DeltaWidth}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack  {DOI Main / \\ \si{\second}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=4, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};
	
\end{axis}

\renewcommand{\NumPlotY}{2}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack { P2M / \\ \si{\micro\second}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=6, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};
\end{axis}

\renewcommand{\NumPlotY}{3}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xticklabel style={/pgf/number format/fixed},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	xticklabels = {},
	xlabel style={font=\color{white!15!black}},
	xlabel={},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={ \shortstack  { SOI Main / \\ \si{\degreeKWbZOT}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=7, col sep=comma] {Figures/Data/MPCData_MCRL_0010MP0004.csv};
\end{axis}



\renewcommand{\NumPlotY}{4}
\pgfmathsetlength{\Ypos}{-1*\NumPlotY*\PlotHeight - 1*\NumPlotY*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(\Xpos, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=2000,
	xlabel style={font=\color{white!15!black}},
	xlabel={Cycle / -},
	xtick={250, 500, 750, 1000, 1250, 1500, 1750},
	ylabel style={at={(-0.1,0.5)}},
	ylabel={\shortstack  {DOI H2 / \\ \si{\second}}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	]
	%\addplot[ area legend, draw=black, fill=blue, opacity=0.5]
	%	table[x index=0, y index=1, col sep=comma]{Figures/Data/PlotEpisode/LimitsRLVSR30089_episode114.csv};
	
	\addplot[ color=mmpDarkBlue,line width=0.5pt,forget plot] table [x index=0, y index=5, col sep=comma]		 {Figures/Data/MPCData_MCRL_0010MP0004.csv};
\end{axis}




\end{tikzpicture}


==> Figures/PlotReward.tex <==
\begin{tikzpicture}
\setlength{\PlotWidth}{6cm} % Example width
\setlength{\PlotHeight}{3.5cm} % Example height
\setlength{\DeltaHeight}{1cm}
\newcommand{\NumPlot}{1}
\pgfmathsetlength{\Ypos}{-1*\NumPlot*\PlotHeight - 1*\NumPlot*\DeltaHeight}
\begin{axis}[%
	width=\PlotWidth,
	height=\PlotHeight,
	at={(0cm, \Ypos)},
	scale only axis,
	xmin=0,
	xmax=20,
	ymin=-3000,
	ymax=0,
	xticklabel style={/pgf/number format/fixed},
	xlabel style={font=\color{white!15!black}},
	xlabel={Groups of $2{.}000$ Cycles / -},
	ylabel={$\sum r$ / -},
    ytick={-2000,-1000,0},
	yticklabels={$-2{.}000$,$-1{.}000$,$0$},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={at={(0.95,0.05)},legend columns=1, legend cell align=left, align=left, anchor=south east,  draw=black,fill=white},
	label style={font=\scriptsize},
	tick label style={font=\scriptsize},
	legend style={font=\scriptsize}
	]
	\addplot[ color=mmpBlack,line width=1pt] table [x index=0, y index=1, col sep=comma] {Figures/Data/RewardVSR1000Groups10.csv};
	\addlegendentry{Overall}
	
\end{axis}



%\renewcommand{\NumPlot}{2}
%\pgfmathsetlength{\Ypos}{-1*\NumPlot*\PlotHeight - 1*\NumPlot*\DeltaHeight}
%\begin{axis}[%
%	width=\PlotWidth,
%	height=\PlotHeight,
%	at={(0cm, \Ypos)},
%	scale only axis,
%	xmin=0,
%	xmax=10,
%	xlabel style={font=\color{white!15!mmpBlack}},
%	xlabel={\gls{rDPMAX} / $\frac{\si{\bar}}{\si{\degreeKW}}$},
%	ymin=0,
%	ymax=27,
%	ylabel style={font=\color{white!15!mmpBlack}},
%	ylabel={Probability / \%},
%	axis background/.style={fill=white},
%	%xmajorgrids,
%	ymajorgrids,
%	legend style={at={(0.96,0.9)},legend columns=1, legend cell align=left, align=left, anchor=north east,  draw=black,fill=white},
%	label style={font=\scriptsize},
%	tick label style={font=\scriptsize},
%	legend style={font=\scriptsize}
%	]
%	
%
%	
%	\addplot[ybar, bar width=0.25, fill=mmpLightGray, draw=mmpBlack, area legend, line width = 0.5] table[row sep=crcr] {%
%        0.125   0.4\\
%		0.625   25.6\\
%		1.125   5.8\\
%		1.625   7.2\\
%		2.125   7.3\\
%		2.625   8.8\\
%		3.125   8.7\\
%		3.625   8.1\\
%		4.125   7.9\\
%		4.625   6.3\\
%		5.125   4.5\\
%		5.625   3.4\\
%		6.125   2\\
%		6.625   2\\
%		7.125   1.4\\
%		7.625   0.4\\
%		8.125   0\\
%		8.625   0\\
%		9.125   0.1\\
%		9.625   0.1\\
%	};
%	\addlegendentry{Group 1}
%	
%	\addplot[ybar, bar width=0.25, fill=mmpDarkGray, draw=mmpBlack, area legend, line width = 0.5] table[row sep=crcr] {%
%        0.375   0.0276\\
%		0.875   6.1641\\
%		1.375   10.4315\\
%		1.875   11.9461\\
%		2.375   16.8496\\
%		2.875   16.6948\\
%		3.375   13.9734\\
%		3.875   10.6888\\
%		4.375   6.6590\\
%		4.875   3.4296\\
%		5.375   1.5806\\
%		5.875   0.7208\\
%		6.375   0.3887\\
%		6.875   0.2002\\
%		7.375   0.1151\\
%		7.875   0.0678\\
%		% Additional data points
%		8.375   0.0384\\
%		8.875   0.0112\\
%		9.375   0.0103\\
%		9.875   0.0023\\
%	};
%	\addlegendentry{Overall}
%
%	
%	   % Plot a vertical line at x=5 from y=0 to y=30
%	\addplot[mmpRed, line width=1pt, domain=0:30, samples=2] coordinates {(5,0) (5,30)};
%	\addlegendentry{$\gls{rDPMAXLim}$}
%	
%	%\node at (axis cs:5,15) {\scriptsize 1. Gruppe von \\ 1000 Zyklen};
%	
%\end{axis}


\end{tikzpicture}


==> Settings/symbols.tex <==
%% ############################ Erklärung ##########################################
% Bei der Definition von Abkürzungen, Symbolen, Akronymen den Identifier
% mit den Buchstaben G, R, A, K (egal ob groß oder klein geschrieben) beginnen
% lassen. Dann sortiert das Glossaries Paket die Einträge korrekt ein. Soll
% heißen: unter die passenden, mit Überschriften versehenden, Abschnitte des
% Abkürzungs- bzw. Symbolverzeichnisses.
% G: Symbol, griechisch - \alpha, \beta, ...
% R: Symbol, lateinisch - A_{\text{Start}}, B_{\text{Gesamt}}, ...
% K: Akronyme - CDU, ADAC, ...
% A: Abkürzungen, allgemein - z.B., usw., ...
% A: Symbol, allgemein - \nabla, \angle

%% Einträge des Symbolverzeichnisses
% Der erste Buchstabe im Index gibt an wo der Eintrag einsortiert werden soll:
% a - Allgemein
% r - Römisches Zeichen
% g - griechisches Zeichen



%% ############################ Defintion ##########################################

%% Allgemeine Symbole
\newglossaryentry{aNabla}{type=symver,name={\ensuremath{\nabla}},description={Nabla Operator},sort={aNabla}}

%% Lateinische Zeichen
%A
\newglossaryentry{rAK}{type=symver,name={\ensuremath{A_\text{K}}},description={Kolbenquerschnittsfläche},sort={iAK}}
\newglossaryentry{rAW}{type=symver,name={\ensuremath{A_\text{W}}},description={Für den Wandwämeübergang wirksame Wandfläche},sort={iAW}}
\newglossaryentry{roNeuron}{type=symver,name={\ensuremath{a}},description={Aktivierungszustand eines künstlichen Neurons},sort={iaNeuron}}

%B
\newglossaryentry{rb}{type=symver,name={\ensuremath{b}},description={Bias-Wert},sort={ib}}

%C
\newglossaryentry{rcv}{type=symver,name={\ensuremath{c_\text{v}}},description={Isochore spezifische Wärmekapazität},sort={icv}}
\newglossaryentry{rCK}{type=symver,name={\ensuremath{K}},description={Menge aller Klassen},sort={iKKlasse}}
\newglossaryentry{rCapacity}{type=symver,name={\ensuremath{C}},description={Elektrische Kapazität},sort={iCapacity}}

%d
\newglossaryentry{rd}{type=symver,name={\ensuremath{d}},description={Abstand},sort={id}}
\newglossaryentry{rdRL}{type=symver,name={\ensuremath{d}},description={Boolescher Indikator für das Ende einer Episode},sort={idaRL}}

\newglossaryentry{rDPMAX}{type=symver,name={\ensuremath{\mathrm{d}\gls{rp}_{\gls{imax}}}},description={Maximaler Druckgradient},sort={iDPMAX}}

\newglossaryentry{rDPMAXi}{type=symver,name={\ensuremath{\mathrm{d}\gls{rp}_{\gls{imax},i}}},description={Maximaler Druckgradient},sort={iDPMAXi}}
\newglossaryentry{rDPMAXi1}{type=symver,name={\ensuremath{\mathrm{d}\gls{rp}_{\gls{imax},i-1}}},description={Maximaler Druckgradient},sort={iDPMAXi1}}
\newglossaryentry{rDPMAXLim}{type=symver,name={\ensuremath{\mathrm{d}\gls{rp}_{\gls{imax},\gls{iLim}}}},description={Maximaler Druckgradient},sort={iDPMAX}}


\newglossaryentry{rDUIONMAX}{type=symver,name={\ensuremath{\mathrm{d}\gls{rUIon}_{,\gls{imax}}}},description={Maximaler Gradient des Ionenstromsignals},sort={iDUIONMAX}}
%E
\newglossaryentry{rEEnergie}{type=symver,name={\ensuremath{E}},description={Energie},sort={iEAEnergie}}
\newglossaryentry{rE}{type=symver,name={\ensuremath{E}},description={Fehler},sort={iE}}
\newglossaryentry{rErr}{type=symver,name={\ensuremath{\mathcal{L}}},description={Fehlerfunktion},sort={iLErr}}
\newglossaryentry{rERL}{type=symver,name={\ensuremath{\mathcal{E}}},description={Episode},sort={iERL}}


%G
\newglossaryentry{rG}{type=symver,name={\ensuremath{G}},description={Ertrag (engl.: Return)},sort={iG}}

%H
\newglossaryentry{rHU}{type=symver,name={\ensuremath{\text{LCV}}},description={Unterer Heizwert},sort={iHU}}
\newglossaryentry{rHUKr}{type=symver,name={\ensuremath{\text{LCV}_{\gls{iKr}}}},description={Unterer Heizwert Kraftstoff},sort={iHU}}
\newglossaryentry{rHUEth}{type=symver,name={\ensuremath{\text{LCV}_{\gls{iEth}}}},description={Unterer Heizwert Ethanol},sort={iHU}}



\newglossaryentry{rHEin}{type=symver,name={\ensuremath{H_{\text{ein}}}},description={Enthalpie des Eingangsmassenstroms},sort={iHEin}}
\newglossaryentry{rHAus}{type=symver,name={\ensuremath{H_{\text{aus}}}},description={Enthalpie des Ausgangsmassenstroms},sort={iHAus}}
\newglossaryentry{rHv}{type=symver,name={\ensuremath{H_{\text{v}}}},description={Verdampfungsenthalpie},sort={iHv}}



%I
\newglossaryentry{rIIon}{type=symver,name={\ensuremath{i_\text{Ion}}},description={Ionenstrom},sort={iIIon}}

\newglossaryentry{rIonMax}{type=symver,name={\ensuremath{\ensuremath{U_{\text{Ion},\gls{imax}}}}},description={Maximum des Ionenstromsignals},sort={iUIonMax}}
\newglossaryentry{rIonMaxi}{type=symver,name={\ensuremath{\ensuremath{U_{\text{Ion},\gls{imax},i}}}},description={Maximum des Ionenstromsignals},sort={iUIonMax}}
\newglossaryentry{rIonMaxi1}{type=symver,name={\ensuremath{\ensuremath{U_{\text{Ion},\gls{imax},i-1}}}},description={Maximum des Ionenstromsignals},sort={iUIonMax}}
\newglossaryentry{rIonIntegral}{type=symver,name={\ensuremath{I_{U_{\text{Ion}}}}},description={Integral des Ionenstroms},sort={iIonIntegral}}
\newglossaryentry{rIonIntegrali}{type=symver,name={\ensuremath{I_{U_{\text{Ion}},i}}},description={Integral des Ionenstroms},sort={iIonIntegral}i}
\newglossaryentry{rIonIntegrali1}{type=symver,name={\ensuremath{I_{U_{\text{Ion}},i-1}}},description={Integral des Ionenstroms},sort={iIonIntegral}i1}



\newglossaryentry{rI}{type=symver,name={\ensuremath{\ensuremath{I}}},description={Relative Wichtigkeit eines Eingangsmerkmals},sort={iI}}

%K
\newglossaryentry{rKP}{type=symver,name={\ensuremath{K_\text{P}}},description={Proportionalanteil eines Reglers},sort={iKP}}



%M
\newglossaryentry{rm}{type=symver,name={\ensuremath{m}},description={Masse},sort={im}}

%N
\newglossaryentry{rnumber}{type=symver,name={\ensuremath{n}},description={Anzahl},sort={inb}}
\newglossaryentry{rNMot}{type=symver,name={\ensuremath{n_\text{Mot}}},description={Motordrehzahl},sort={inMot}}
\newglossaryentry{rni}{type=symver,name={\ensuremath{n_i}},description={Stoffmenge einer Komponente $i$},sort={ini}}

\newglossaryentry{rNG}{type=symver,name={\ensuremath{\mathcal{N}}},description={Gaußsches Rauschen},sort={iNA}}

%O
\newglossaryentry{rO}{type=symver,name={\ensuremath{\boldsymbol{O}}},description={Orientierungsmatrix des Vermessungsalgorithmus},sort={iO}}
\newglossaryentry{ro}{type=symver,name={\ensuremath{o}},description={Element der Orientierungsmatrix},sort={iO}}

%P
\newglossaryentry{rp}{type=symver,name={\ensuremath{p}},description={Druck},sort={ip}}
%\newglossaryentry{rpmi}{type=symver,name={\ensuremath{p_{\text{mi}}}},description={Indizierter Mitteldruck},sort={ipmi}}
%\newglossaryentry{rpmii} {type=symver,name={\ensuremath{p_{\text{mi},i}}},description={Indizierter Mitteldruck},sort={ipmii}}
%\newglossaryentry{rpmii1} {type=symver,name={\ensuremath{p_{\text{mi},i-1}}},description={Indizierter Mitteldruck},sort={ipmii1}}
%\newglossaryentry{rpmiSoll} {type=symver,name={\ensuremath{p_{\text{mi},\gls{iSoll}}}},description={Indizierter Mitteldruck},sort={ipmiSoll}}
%\newglossaryentry{rpmiiSoll} {type=symver,name={\ensuremath{p_{\text{mi},\gls{iSoll},i}}},description={Indizierter Mitteldruck},sort={ipmiiSoll}}
%\newglossaryentry{rpmii1Soll} {type=symver,name={\ensuremath{p_{\text{mi},\gls{iSoll},i-1}}},description={Indizierter Mitteldruck},sort={ipmii1Soll}}

\newglossaryentry{rpmi}{type=symver,name={\ensuremath{\text{IMEP}}},description={Indizierter Mitteldruck},sort={ipmi}}
\newglossaryentry{rpmii}
{type=symver,name={\ensuremath{\text{IMEP}_{i}}},description={Indizierter Mitteldruck},sort={ipmii}}
\newglossaryentry{rpmii1}
{type=symver,name={\ensuremath{\text{IMEP}_{i-1}}},description={Indizierter Mitteldruck},sort={ipmii1}}
\newglossaryentry{rpmiSoll}
{type=symver,name={\ensuremath{\text{IMEP}_{\gls{iSoll}}}},description={Indizierter Mitteldruck},sort={ipmiSoll}}
\newglossaryentry{rpmiiSoll}
{type=symver,name={\ensuremath{\text{IMEP}_{\gls{iSoll},i}}},description={Indizierter Mitteldruck},sort={ipmiiSoll}}
\newglossaryentry{rpmii1Soll}
{type=symver,name={\ensuremath{\text{IMEP}_{\gls{iSoll},i-1}}},description={Indizierter Mitteldruck},sort={ipmii1Soll}}


\newglossaryentry{rP}{type=symver,name={\ensuremath{P}},description={Wahrscheinlichkeit},sort={iP}}

%Q
\newglossaryentry{rQ}{type=symver,name={\ensuremath{Q}},description={Wärmefreisetzung durch Verbrennung},sort={iQW}}
\newglossaryentry{rQW}{type=symver,name={\ensuremath{Q_\text{W}}},description={Wandwärmeverluste},sort={iQZ}}
\newglossaryentry{rQfunc}{type=symver,name={\ensuremath{Q}},description={Q-Funktion},sort={iQA}}

%R
\newglossaryentry{rRGas}{type=symver,name={\ensuremath{R}},description={Universelle Gaskonstante},sort={iRU}}
\newglossaryentry{rRShunt}{type=symver,name={\ensuremath{R_\text{Shunt}}},description={Einstellbarer Widerstand zur Messung des Ionenstroms},sort={iRE}}
\newglossaryentry{rr}{type=symver,name={\ensuremath{R}},description={Radius des Vermessungsalgorithmus},sort={iRR}}
\newglossaryentry{rRVermessung}{type=symver,name={\ensuremath{R}},description={Positionsmatrix des Vermessungsalgorithmus},sort={iRM}}

\newglossaryentry{rRReward}{type=symver,name={\ensuremath{r}},description={Belohnung (engl.: Reward)},sort={irzb}}
\newglossaryentry{rrDeltaExpl}{type=symver,name={\ensuremath{\Delta r_\text{Expl}}},description={Schrittweite des Vermessungsalgorithmus in radialer Richtung},sort={irzz}}
\newglossaryentry{rrCor}{type=symver,name={\ensuremath{r}},description={Korrelationskoeffizient},sort={irzk}}

\newglossaryentry{rRMSE}{type=symver,name={\text{RMSE}},description={Root Mean Square Error},sort={rRMSE}}


%S
\newglossaryentry{rs}{type=symver,name={\ensuremath{s}},description={Iterationsschritt},sort={is}}

%T

\newglossaryentry{rT}{type=symver,name={\ensuremath{T}},description={Temperatur},sort={iTA}}
\newglossaryentry{rTRL}{type=symver,name={\ensuremath{T}},description={Tupel einer  Erfahrung beim Reinforcement Learning},sort={iTB}}

\newglossaryentry{rt}{type=symver,name={\ensuremath{t}},description={Zeit},sort={itB}}
\newglossaryentry{rTWand}{type=symver,name={\ensuremath{T_\text{W}}},description={Wandtemperatur},sort={iTWand}}




%U

\newglossaryentry{rURaum}{type=symver,name={\ensuremath{\mathcal{A}}},description={Aktionsraum},sort={iU}}

\newglossaryentry{rU}{type=symver,name={\ensuremath{U}},description={Innere Energie},sort={iUA}}

\newglossaryentry{ru}{type=symver,name={\ensuremath{u}},description={spezifische innere Energie},sort={iua}}

\newglossaryentry{ruCtrl}{type=symver,name={\ensuremath{a}},description={Stellgröße},sort={iub}}

\newglossaryentry{ruCtrlVec}{type=symver,name={\ensuremath{\vec{a}}},description={Vektor der Stellgrößen},sort={iuc}}

\newglossaryentry{rUDC}{type=symver,name={\ensuremath{U_\text{dc}}},description={Angelegte Gleichspannung zur Bestimmung des Ionenstroms},sort={iud}}

\newglossaryentry{rUIon}{type=symver,name={\ensuremath{U_\text{Ion}}},description={Ionenstrom gemessen als Spannungsabfall},sort={iue}}

%U
%\newglossaryentry{rUASafeNorm}{type=symver,name={\ensuremath{u_{\text{A,Safe,Norm}}}},description={Sichere, normierte Aktion nach Überprüfung durch Überwachungsfunktion},sort={iUASafeNorm}}
%\newglossaryentry{rUA}{type=symver,name={\ensuremath{u_\text{A}}},description={Aktion des Agenten},sort={iUA}}
%\newglossaryentry{rUAMin}{type=symver,name={\ensuremath{u_\text{A,min}}},description={Minimal erlaubte Aktion des Agenten},sort={iUAMin}}
%\newglossaryentry{rUAMax}{type=symver,name={\ensuremath{u_\text{A,max}}},description={Maximal erlaubte Aktion des Agenten},sort={iUAMax}}
%\newglossaryentry{rUARoh}{type=symver,name={\ensuremath{u_\text{A,Roh}}},description={Reellwertige Rohaktion des Agenten},sort={iUARoh}}




%V

\newglossaryentry{rV}{type=symver,name={\ensuremath{V}},description={Volumen},sort={iVA}}
\newglossaryentry{rVRL}{type=symver,name={\ensuremath{V}},description={Wertefunktion},sort={iVB}}

\newglossaryentry{rRichtungsvektor}{type=symver,name={\ensuremath{\vec{v}}},description={Richtungsvektor des Vermessungsalgorithmus},sort={ivC}}

\newglossaryentry{rVC}{type=symver,name={\ensuremath{V_{\mathrm{C}}}},description={kompressionsvolumen},sort={iVD}}
\newglossaryentry{rVH}{type=symver,name={\ensuremath{V_{\mathrm{H}}}},description={Hubvolumen},sort={iVE}}
\newglossaryentry{rvkm}{type=symver,name={\ensuremath{v_\text{K,m}}},description={Mittlere Kolbengeschwindigkeit},sort={ivF}}



%W
\newglossaryentry{rWK}{type=symver,name={\ensuremath{W_{\mathrm{K}}}},description={Volumenarbeit am Kolben},sort={iWc}}
\newglossaryentry{rW}{type=symver,name={\ensuremath{W}},description={Arbeit},sort={iWA}}
\newglossaryentry{rw}{type=symver,name={\ensuremath{w}},description={Gewichtung},sort={iwb}}

%X

\newglossaryentry{rX}{type=symver,name={\ensuremath{\mathcal{S}}},description={Zustandsraum},sort={iX}}

\newglossaryentry{rxAnteil}{type=symver,name={\ensuremath{x}},description={Anteil},sort={ixA}}


\newglossaryentry{rxState}{type=symver,name={\ensuremath{s}},description={Zustandsgröße},sort={ixb}}

\newglossaryentry{rxStateVec}{type=symver,name={\ensuremath{\vec{s}}},description={Vektor der Zustandsgrößen},sort={ixc}}

\newglossaryentry{rxAbg}{type=symver,name={\ensuremath{x_{\mathrm{abg}}}},description={Abgasrückführrate},sort={ixd}}




%Z
\newglossaryentry{rZ}{type=symver,name={\ensuremath{\boldsymbol{Z}}},description={Zählermatrix des Vermessungsalgorithmus},sort={iZA}}

\newglossaryentry{rz}{type=symver,name={\ensuremath{z}},description={Element der Zählermatrix},sort={izb}}

\newglossaryentry{rnet}{type=symver,name={\ensuremath{z}},description={Nettoeingabewert eines künstlichen Neurons},sort={izc}}


%% Griechische Zeichen
%Reihenfolge: Alpha(a), Beta(b), Gamma(c), Delta(d), Epsilon(e), Zeta(f), Eta(g), Theta(h), Iota(i), Kappa(j), Lambda(k), Mu(l), Nu(m), Xi(n), Omikron(o), Pi(p), Rho(q), Sigma(r), Tau(s), Ypsilon(t), Phi(u), Chi(v), Psi(w), Omega(x)

%alpha
\newglossaryentry{gAlpha}{type=symver,name={\ensuremath{\alpha}},description={Kurbelwinkel},sort={ga}}
\newglossaryentry{gAlpha50}{type=symver,name={\ensuremath{\alpha_{50}}},description={Verbrennungsschwerpunktlage},sort={ga50}}
\newglossaryentry{gAlpha50i}{type=symver,name={\ensuremath{\alpha_{50,i}}},description={Verbrennungsschwerpunktlage},sort={ga50i}}
\newglossaryentry{gAlpha50i1}{type=symver,name={\ensuremath{\alpha_{50,i-1}}},description={Verbrennungsschwerpunktlage},sort={ga50i1}}
\newglossaryentry{gAlpha50Soll}{type=symver,name={\ensuremath{\alpha_{50,\gls{iSoll}}}},description={Verbrennungsschwerpunktlage},sort={ga50Soll}}



\newglossaryentry{gAlphaIon50}{type=symver,name={\ensuremath{\alpha_{\text{Ion},50}}},description={Winkel bei dem 50 \% des Ionenstromintegrals erreicht sind},sort={ga50Ion}}
\newglossaryentry{gAlphaK}{type=symver,name={\ensuremath{\alpha_\text{K}}},description={Durchströmzahl},sort={gak}}
\newglossaryentry{gAlphaW}{type=symver,name={\ensuremath{\alpha_\text{W}}},description={Wärmeübergangskoeffizient},sort={gaw}}
%gamma
\newglossaryentry{ggamma}{type=symver,name={\ensuremath{\gamma}},description={Diskontierungsfaktor},sort={gc}}
%epsilon
\newglossaryentry{gepsilon}{type=symver,name={\ensuremath{\varepsilon}},description={Verdichtungsverhältnis},sort={ge}}
%eta
\newglossaryentry{geta}{type=symver,name={\ensuremath{\eta_\text{i}}},description={Indizierter Wirkungsgrad},sort={gg}}
%theta
\newglossaryentry{gtheta}{type=symver,name={\ensuremath{\theta}},description={Schwellenwert einer Aktivierungsfunktion},sort={ghSchwellenwert}}
\newglossaryentry{gthetaParam}{type=symver,name={\ensuremath{\theta}},description={Parameter des Parametersatzes \gls{gTheta}},sort={ghParam}}
\newglossaryentry{gTheta}{type=symver,name={\ensuremath{\Theta}},description={Parametersatz eines neuronalen Netzes},sort={gH}}
%kappa
\newglossaryentry{gKappa}{type=symver,name={\ensuremath{\kappa}},description={Isentropenexponent},sort={gj}}
%lambda
\newglossaryentry{gLambda}{type=symver,name={\ensuremath{\lambda_{\text{L}}}},description={Kraftstoff-Luft-Verhältnis},sort={gkbLambda}}
\newglossaryentry{gLambdaRL}{type=symver,name={\ensuremath{\lambda}},description={Abklingfaktor},sort={gkaLambdaRL}}

%Mu
\newglossaryentry{gm}{type=symver,name={\ensuremath{\mu}},description={Mittelwert einer Verteilung},sort={glaM}}
\newglossaryentry{gmRL}{type=symver,name={\ensuremath{\mu}},description={Deterministische Strategie eines Reinforcement Learning-Agenten},sort={glaD}}
\newglossaryentry{gmi}{type=symver,name={\ensuremath{\mu_i}},description={Chemisches Potenzial einer Komponente $i$},sort={glb}}

%rho
\newglossaryentry{grho}{type=symver,name={\ensuremath{\rho}},description={Dichte},sort={gq}}
\newglossaryentry{grhoPoly}{type=symver,name={\ensuremath{\rho}},description={Faktor für die Mittelung nach Polyak},sort={gqPoly}}
%sigma
\newglossaryentry{gsigma}{type=symver,name={\ensuremath{\sigma}},description={Empirische Standardabweichung},sort={gr}}
\newglossaryentry{gsigmaP}{type=symver,name={\ensuremath{\sigma}},description={Propagierungsfunktion},sort={grP}}
%PHI
\newglossaryentry{gphi}{type=symver,name={\ensuremath{\varphi}},description={Aktivierungsfunktion},sort={gu}}
\newglossaryentry{gPhi}{type=symver,name={\ensuremath{\varPhi}},description={Wahrscheinlichkeitsdichte},sort={gU}}

%Pi
\newglossaryentry{gpi}{type=symver,name={\ensuremath{\pi}},description={Stochastische Strategie eines Reinforcement Learning-Agenten},sort={gp}}

%psi
\newglossaryentry{gpsi}{type=symver,name={\ensuremath{\psi}},description={Durchflussfunktion},sort={gw}}

%xi
\newglossaryentry{gxi}{type=symver,name={\ensuremath{\xi}},description={Lernrate},sort={gn}}


%Indizes
%A
\newglossaryentry{iA}{type=symver,name={\ensuremath{\text{A}}},description={Ausgabeschicht eines künstlichen neuronalen Netzes},sort={rA}}
\newglossaryentry{iAbg}{type=symver,name={\ensuremath{\text{Abg}}},description={Abgas},sort={rAbg}}
%B
\newglossaryentry{iBatch}{type=symver,name={\ensuremath{b}},description={\gls{iBatch}-tes Element eines Mini-Batches},sort={rBatch}}

%D
\newglossaryentry{iDMV}{type=symver,name={\ensuremath{\text{DMV}}},description={Größe der dynamischen Multiskalenvermessung},sort={rDMV}}

%E
\newglossaryentry{iEth}{type=symver,name={\ensuremath{\text{Eth}}},description={Ethanol},sort={rEth}}
\newglossaryentry{iEnde}{type=symver,name={\ensuremath{\text{Ende}}},description={Ende eines Intervalls},sort={rEnde}}
%I
\newglossaryentry{iZyklus}{type=symver,name={\ensuremath{i}},description={\gls{iZyklus}-ter Verbrennungszyklus},sort={rib}}

\newglossaryentry{iiNeuron}{type=symver,name={\ensuremath{i}},description={\gls{iiNeuron}-tes Eingabeneuron},sort={ria}}

\newglossaryentry{iInj}{type=symver,name={\ensuremath{\text{Inj}}},description={Einspritzung},sort={ric}}

%J
\newglossaryentry{ij}{type=symver,name={\ensuremath{j}},description={\gls{ij}-te Stellgröße},sort={rjb}}
\newglossaryentry{ijNeuron}{type=symver,name={\ensuremath{j}},description={\gls{ijNeuron}-tes Ausgabeneuron},sort={rja}}

\newglossaryentry{ijParam}{type=symver,name={\ensuremath{j}},description={\gls{ijParam}-ter Paramter der Fehlerfunktion \gls{rErr}},sort={rjParam}}
%K
\newglossaryentry{iK}{type=symver,name={\ensuremath{\text{K}}},description={Kühlwasser},sort={rK}}
\newglossaryentry{iKr}{type=symver,name={\ensuremath{\text{Gas}}},description={Kraftstoff},sort={rKr}}
\newglossaryentry{iKlasse}{type=symver,name={\ensuremath{k}},description={\gls{iKlasse}-te Klasse des Vermessungsalgorithmus},sort={rk}}
%L
\newglossaryentry{iL}{type=symver,name={\ensuremath{\text{L}}},description={Luft},sort={rL}}
\newglossaryentry{iLW}{type=symver,name={\ensuremath{\text{LW}}},description={Ladungswechsel},sort={rLW}}
\newglossaryentry{iLim}{type=symver,name={\ensuremath{\text{Lim}}},description={Limit},sort={rLim}}
\newglossaryentry{iVZyklus}{type=symver,name={\ensuremath{m}},description={\gls{iVZyklus}-ter Vermessungszyklus},sort={rm}}
\newglossaryentry{ilayer}{type=symver,name={\ensuremath{l}},description={\gls{ilayer}-te Schicht eines künstlichen neuronalen Netzes},sort={rlayer}}


%M
\newglossaryentry{iRichtung}{type=symver,name={\ensuremath{l}},description={\gls{iRichtung}-te Richtung der Vermessung},sort={rl}}
\newglossaryentry{imax}{type=symver,name={\ensuremath{\text{Max}}},description={Maximum},sort={rmax}}
\newglossaryentry{imin}{type=symver,name={\ensuremath{\text{Min}}},description={Minimum},sort={rmin}}
%N
\newglossaryentry{iNorm}{type=symver,name={\ensuremath{\text{Norm}}},description={Normalisierte Größe},sort={rNorm}}
\newglossaryentry{iN}{type=symver,name={\ensuremath{\text{N}}},description={Nachbarn},sort={rN}}
\newglossaryentry{iNVO}{type=symver,name={\ensuremath{\text{NVO}}},description={Negative Ventilüberschneidung (engl.: negative Valve Overlap)},sort={rNVO}}

%H
\newglossaryentry{iHD}{type=symver,name={\ensuremath{\text{HD}}},description={Hochdruckprozess},sort={rHD}}



%K
\newglossaryentry{ikomp}{type=symver,name={\ensuremath{\text{Komp}}},description={Kompensation},sort={rkomp}}


\newglossaryentry{iKNN}{type=symver,name={\ensuremath{\text{KNN}}},description={Künstliches neuronales Netz},sort={rKNN}}

%O
\newglossaryentry{iOl}{type=symver,name={\ensuremath{\text{Öl}}},description={Öl},sort={rOl}}
%S
\newglossaryentry{iSoll}{type=symver,name={\ensuremath{\text{Set}}},description={Sollgröße},sort={rSoll}}
\newglossaryentry{iSchw}{type=symver,name={\ensuremath{\text{Schw}}},description={Aktivierungsschwelle},sort={rSchw}}
\newglossaryentry{iSau}{type=symver,name={\ensuremath{\text{Sau}}},description={Saugrohr},sort={rSau}}
\newglossaryentry{iStartInt}{type=symver,name={\ensuremath{\text{Start}}},description={Start eines Intervalls},sort={rStartInt}}
\newglossaryentry{iStart}{type=symver,name={\ensuremath{\text{Start}}},description={Startpunkt der Vermessung},sort={rStart}}
%U
\newglossaryentry{iU}{type=symver,name={\ensuremath{\text{U}}},description={Umgebung},sort={rU}}
\newglossaryentry{iUnsicher}{type=symver,name={\ensuremath{\text{Unsafe}}},description={Unsafe state},sort={rUnsicher}}
\newglossaryentry{iSafetyFilter}{type=symver,name={\ensuremath{\text{Safety}}},description={Safety},sort={rUberwachung}}

% R
\newglossaryentry{iRL}{type=symver,name={\ensuremath{\text{RL}}},description={Größe des Reinforcement Learning-Agenten},sort={rRL}}
\newglossaryentry{iRoh}{type=symver,name={\ensuremath{\text{Raw}}},description={Rohwert},sort={rRoh}}
%S
\newglossaryentry{iSicher}{type=symver,name={\ensuremath{\text{Safe}}},description={Safe State},sort={rSicher}}
%T
\newglossaryentry{iTol}{type=symver,name={\ensuremath{\text{Tol}}},description={Toleranz},sort={rTol}}
\newglossaryentry{iTest}{type=symver,name={\ensuremath{\text{Test}}},description={Testdatensatz},sort={rTest}}
\newglossaryentry{iTrain}{type=symver,name={\ensuremath{\text{Train}}},description={Trainingsdatensatz},sort={rTrain}}

%V
\newglossaryentry{iverbrannt}{type=symver,name={\ensuremath{\text{v}}},description={Verbrannt},sort={rvverbrannt}}

%W
\newglossaryentry{iW}{type=symver,name={\ensuremath{\text{W}}},description={Wasser},sort={rW}}
%Z
\newglossaryentry{iZyl}{type=symver,name={\ensuremath{\text{cyl}}},description={Zylinder},sort={rZyl}}
\newglossaryentry{iZK}{type=symver,name={\ensuremath{\text{ZK}}},description={Zwischenkompression},sort={rZK}}

